Early Risk Prediction of Pediatric Cardiac Arrest from Electronic Health Records via Multimodal Fused Transformer

Early prediction of pediatric cardiac arrest (CA) is critical for timely intervention in high-risk intensive care settings. We introduce PedCA-FT, a novel transformer-based framework that fuses tabular view of EHR with the derived textual view of EHR to fully unleash the interactions of high-dimensional risk factors and their dynamics. By employing dedicated transformer modules for each modality view, PedCA-FT captures complex temporal and contextual patterns to produce robust CA risk estimates. Evaluated on a curated pediatric cohort from the CHOA-CICU database, our approach outperforms ten other artificial intelligence models across five key performance metrics and identifies clinically meaningful risk factors. These findings underscore the potential of multimodal fusion techniques to enhance early CA detection and improve patient care.

==> sections/related_work.tex <==
\section{Related Work}
% !!!Not used for 7-page submission EMBC!!!
\subsection{Electronic Health Records Based Risk Prediction}
EHR is a valuable resource for patient risk prediction, and has been widely used for many adverse health events, including but not limited to cardiac arrest~\cite{do2019usefulness,brown2025MLCA}, mortality~\cite{wornow2023ehrshot}, re-hospitalization~\cite{shao2025SDOH-mine}. 
Although EHRs provide a rich collection of patient information, their utilization in risk prediction remains challenging. 
This is primarily due to (1) the heterogeneous nature of the tabular data ranging from numerical vital signs and lab results to categorical demographics and diagnosis; and (2) the multi-resolution characteristics inherent to these longitudinal records where vital signs might be recorded every few minutes while lab results are typically updated only a few times per day. Such variability in data~\cite{zeng2020pic}, combined with issues like missing data and noise, requires sophisticated preprocessing~\cite{wornow2023ehrshot,brown2025MLCA}, integration, and modeling techniques to effectively capture and analyze the underlying temporal and clinical patterns. Therefore, the development of robust EHR-based risk prediction systems demands advanced data fusion methods~\cite{lu2023mug} that can seamlessly manage the complexities of heterogeneous and multi-resolution data.


\subsection{AI Models for Pediatric Cardiac Arrest Prediction}
AI models have been increasingly explored for pediatric cardiac arrest prediction to enhance early detection and intervention, leveraging different combination of data reside in EHRs. 
%Due to the variable recording frequencies of different data (\textit{e.g.} vital signs routinely recorded every several minutes, lab test taken every several hours), researchers have came up with different approaches to handle the heterogenity. 
Due to the heterogeneity and multi-resolution property of EHR, .
The most straightforward approach is to aggregate the multi-resolution time-series features into summarized representation via aggregation operations (\textit{e.g.} $\text{MAX}(\cdot)$, $\text{AVERAGE}(\cdot)$, $\text{LAST}(\cdot)$).
Another way is to unify the resolutions into a pre-defined interval (\textit{e.g.} 1 hour), and impute missing data.
%Early exploration to handle the heterogenous multimodal EHR data has been focusing on designing effective scoring tool to fuse major organ system's deterioration (\textit{e.g}. PEWS~\cite{monaghan2005pews}). Uni-modal AI models such as K-nearest neighbor and support vector machine can be utilized to predict CA risk based on the derived deterioration score.


%Early exploration has been focused on utilize mainly one modality of EHR data. For instance, researchers have explored machine learning models (e.g. Rocket~\cite{dempster2021minirocket}) and later time-series foundation models (e.g. Moment~\cite{goswami2024momentfamilyopentimeseries}) to predict CA in advance based on continuous non-invasive electrocardiographic~\cite{do2019usefulness}.
%This includes not only ECG signals but also additional modalities such as patient demographics, vital signs (e.g., peripheral cutaneous oxygen saturation, heart rate, blood pressure), laboratory results, and clinical notes. By fusing these diverse data sources, AI models can potentially capture a broader spectrum of physiological changes and risk factors, thereby improving early warning systems in pediatric critical care.

%Uni-modality models are designed to process static features, making them effective for tasks involving homogeneous numerical data, which can be easily handled by traditional machine learning models such as K-Nearest Neighbor or Linear Regression. However, when dealing with time-series data, certain critical information may be lost—e.g., using the last observed value disregards temporal dynamics. By the same token, some uni-modality models, such as MOMENT\cite{goswami2024momentfamilyopentimeseries}, specifically target temporal relationships, preserving these dynamics and achieving superior performance and adaptability compared to traditional approaches. In contrast, multi-modality models, such as Shapelet\cite{Guillaume_2022} and Rocket\cite{Dempster_2020}, integrate diverse feature types, including static and temporal data, capturing richer contextual information. This enables them to outperform uni-modality models in healthcare settings, where understanding relationships between heterogeneous data sources, such as patient profile (static) and medical signals (temporal), is essential for improved predictive performance.


%\subsection{Sample and Feature Selection Methods}
%LLM-select~\cite{jeong2024llmselect} is a pioneering work that utilize LLM for feature selection, where they propose three prompting strategies: LLM-score, LLM-rank, LLM-seq. LLM-score outputs a feature importance score for each input feature, LLM-rank outputs a ranked list with regards to feature importance, and LLM-seq iteratively generates the included feature list until a pre-defined length. As can be seen, all LLM-select methods require certain pre-defined threshold to determine which features can be included. \jiaying{we can include comparison at Appendix for our llm-fprune v.s. LLM-select.}
